TOFFE -- Temporally-binned Object Flow from Events for High-speed and Energy-Efficient Object Detection and Tracking

Object detection and tracking is an essential perception task for enabling fully autonomous navigation in robotic systems. Edge robot systems such as small drones need to execute complex maneuvers at high-speeds with limited resources, which places strict constraints on the underlying algorithms and hardware. Traditionally, frame-based cameras are used for vision-based perception due to their rich spatial information and simplified synchronous sensing capabilities. However, obtaining detailed information across frames incurs high energy consumption and may not even be required. In addition, their low temporal resolution renders them ineffective in high-speed motion scenarios. Event-based cameras offer a biologically-inspired solution to this by capturing only changes in intensity levels at exceptionally high temporal resolution and low power consumption, making them ideal for high-speed motion scenarios. However, their asynchronous and sparse outputs are not natively suitable with conventional deep learning methods. In this work, we propose TOFFE, a lightweight hybrid framework for performing event-based object motion estimation (including pose, direction, and speed estimation), referred to as Object Flow. TOFFE integrates bio-inspired Spiking Neural Networks (SNNs) and conventional Analog Neural Networks (ANNs), to efficiently process events at high temporal resolutions while being simple to train. Additionally, we present a novel event-based synthetic dataset involving high-speed object motion to train TOFFE. Our experimental results show that TOFFE achieves 5.7x/8.3x reduction in energy consumption and 4.6x/5.8x reduction in latency on edge GPU(Jetson TX2)/hybrid hardware(Loihi-2 and Jetson TX2), compared to previous event-based object detection baselines.

==> Tables/energy_and_latency.tex <==
\begin{table*}[!htp]
    \centering
    \setlength{\tabcolsep}{10pt}
    \renewcommand*{\arraystretch}{1.2}
    \subfloat[Dynamic Energy per Inference ($mJ$)]{
        \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Model} & \multirow{2}{*}{Output} & CPU & GPU & Edge GPU & Hybrid Hardware \\
        & & i9-12700KF & RTX 3090-Ti & Jetson TX2 & Loihi-2 \& Jetson TX2 \\ \hline \hline
        DOTIE (- clustering) \cite{dotie} & Speed Separation & 28.8 & 31.1 & 4.6 & 0.083 \\ \hline
        Adaptive-SpikeNet (Pico) \cite{adaptivespikenet} & Optical Flow & 1029.1 & 417.2 & 89.2 & - \\
        DOTIE \cite{dotie} & Object Detection & 558.0 & 426.9 & 74.2 & - \\
        \rowcolor{LightCyan} \textbf{TOFFE (ours)} & \textbf{Object Flow} & \textbf{92.5} & \textbf{123.0} & \textbf{13.0} & \textbf{0.1302} \\ 
        \hline
        \end{tabular}
    }
    \hfill
    \par\bigskip    
    \subfloat[Inference Rate (samples/sec)]{
        \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Model} & \multirow{2}{*}{Output} & CPU & GPU & Edge GPU & Hybrid Hardware \\
        & & i9-12700KF & RTX 3090-Ti & Jetson TX2 & Loihi-2 \& Jetson TX2 \\ \hline \hline
        DOTIE (- clustering) \cite{dotie} & Speed Separation & 1605.7 & 2938.8 & 168.1 & 3459.5 \\ \hline
        Adaptive-SpikeNet (Pico) \cite{adaptivespikenet} &Optical Flow & 41.6 & 241.7 & 23.9 & - \\
        DOTIE \cite{dotie} & Object Detection & 60.3 & 222.2 & 10.7 &- \\ 
        \rowcolor{LightCyan} \textbf{TOFFE (ours)} & \textbf{Object Flow} & \textbf{460.6} & \textbf{744.6} & \textbf{49.7} & \textbf{201.7} \\ 
        \hline
        \end{tabular}
    }
\captionof{table}{Energy (a) and latency (b) results of SOTA lightweight SNN approaches for object detection, optical flow and combined outputs. We use DOTIE as a baseline as it comprises of a single convolutional operator with LIF neurons (similar to TOFF-E’s OFS SNN component). Best results are bolded.}
\label{tab:energy_and_latency}
\end{table*}

==> Tables/figure1_old.tex <==
\begin{table}[t]
  \centering
  \renewcommand*{\arraystretch}{1.2}
  \begin{tabular}{cccc}
    % Input
    % \begin{minipage}{.176\textwidth}
    %   \includegraphics[width=1.07\textwidth]{Figures/Event_input_bw.png}
    % \end{minipage}
    % & 
    % % Adaptive-spikenet 
    % \begin{minipage}{.176\textwidth}
    %   \includegraphics[width=1.07\textwidth]{Figures/ASPF_for_input/blk_bg_scaled.png}
    % \end{minipage}
    % & 
    % % DOTIE + DBSCAN output
    % \begin{minipage}{.176\textwidth}
    %   \includegraphics[width=1.07\textwidth]{Figures/DOTIE_DBSCAN_for_input_bw.png}
    % \end{minipage}
    % &
    % % MOTE
    % \begin{minipage}{.176\textwidth}
    %   \includegraphics[width=1.07\textwidth]{Figures/Event_input_bw.png}
    % \end{minipage}
    % \\ 
    \textbf{Task} & \textbf{Adaptive-SpikeNet \cite{adaptivespikenet}} & \textbf{DOTIE \cite{dotie}} & \textbf{TOFFE} \\ \hline
  \multicolumn{1}{|c|}{\cellcolor{LightCyan}\textbf{Pose}} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\cmark} \\  
  \multicolumn{1}{|c|}{\cellcolor{LightCyan}\textbf{Direction}} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} \\ 
  \multicolumn{1}{|c|}{\cellcolor{LightCyan}\textbf{Speed}} & \multicolumn{1}{c|}{Exact} & \multicolumn{1}{c|}{Approximate} & \multicolumn{1}{c|}{Approximate} \\ \hline
  % \multicolumn{1}{|c|}{\cellcolor{LightCyan}\textbf{Object Tracking}} & \multicolumn{1}{c|}{\xmark} & \multicolumn{1}{c|}{\cmark} & \multicolumn{1}{c|}{\cmark} \\  \hline
  \end{tabular}
\captionof{figure}{Comparison of TOFFE with Adaptive-spikenet \cite{adaptivespikenet} and DOTIE \cite{dotie} for object flow estimation.}
\label{Fig:all_alg_comparisons}
\vspace{-6mm}
\end{table}

==> Tables/inference_rate.tex <==
% \begin{table*}[!htp]
%     \centering
%     \setlength{\tabcolsep}{21.5pt}
%     \renewcommand*{\arraystretch}{1.25}
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%     Model & \# Params & Output & CPU & GPU & Loihi-2 \\ \hline \hline
%     DOTIE \cite{dotie} & X & Object Tracking & 1606 & 2939 & 3460 \\
%     DOTIE (+ DBSCAN) \cite{dotie} & X &Object Detection & 60 & 222 & N/A \\
%     Adaptive-SpikeNet (Pico) \cite{adaptivespikenet} & X &Optical Flow & 42 & 242 & N/A \\
%     \rowcolor{LightCyan} \textbf{MOTE v0 (ours)} & \textbf{X} & \textbf{Object Flow} & \textbf{571} & \textbf{1130} & \textbf{218} \\ 
%     \hline
%     \end{tabular}
% \captionof{table}{Inference Rate (FPS)}
% \label{tab:inference_rate}
% \end{table*}

% \begin{table*}[!htp]
%     \centering
%     \setlength{\tabcolsep}{15pt}
%     \renewcommand*{\arraystretch}{1.25}
%     \begin{tabular}{|c|c|c|c|c|c|}
%     \hline
%     Model & Output & i9-12700KF & RTX 3090-Ti & Jetson TX2 & Loihi-2 \\ \hline \hline
%     DOTIE \cite{dotie} & Object Tracking & 1605.7 & 2938.8 & 168.1 & 3459.5 \\ \hline
%     DOTIE (+ DBSCAN) \cite{dotie} &Object Detection & 60.3 & 222.2 & 10.7 & N/A \\
%     Adaptive-SpikeNet (Pico) \cite{adaptivespikenet} &Optical Flow & 41.6 & 241.7 & 23.9 & N/A \\
%     \rowcolor{LightCyan} \textbf{TOFF-E (ours)} & \textbf{Object Flow} & \textbf{460.6} & \textbf{744.6} & \textbf{49.7} & \textbf{201.7} \\ 
%     \hline
%     \end{tabular}
% \captionof{table}{Inference Rate ($FPS$)}
% \label{tab:inference_rate}
% \end{table*}

==> Tables/noise_ablation.tex <==
\begin{table*}[!htp]
    \centering
    \setlength{\tabcolsep}{15pt}
    \renewcommand*{\arraystretch}{1.25}
    \subfloat[PSNR]{
        \begin{tabular}{|c|c|c|c|}
        \hline
        Noise Level & Adaptive-SpikeNet~\cite{adaptivespikenet} & DOTIE~\cite{dotie} & TOFFE (This work) \\ \hline \hline
        % 0\% & - & - & -\\ 
        1\% & 39.23 & 36.88 & 42.24\\
        2\% & 38.55 & 35.92 & 39.56 \\
        5\% & 37.88 & 35.08 & 38.42 \\ 
        10\% & 35.27 & 33.24 & 36.62 \\ 
        \hline
        \end{tabular}
    }

    \subfloat[SSIM]{
        \begin{tabular}{|c|c|c|c|}
        \hline
        Noise Level & Adaptive-SpikeNet~\cite{adaptivespikenet} & DOTIE~\cite{dotie} & TOFFE (This work) \\ \hline \hline
        % 0\% & - & - & -\\ 
        1\% & 0.995 & 0.988 & 0.998 \\
        2\% & 0.992 & 0.925 & 0.992 \\
        5\% & 0.985 & 0.882 & 0.987 \\ 
        10\% & 0.971 & 0.722 & 0.968 \\ 
        \hline
        \end{tabular}
    }
    
\captionof{table}{Ablation study with noisy data with different noise levels - 1\%, 2\%, 5\%, 10\%.}
\label{tab:energy_and_latency}
\end{table*}
